Quantum Geometry and Nonlinear Responses in Magnetic and Topological Quantum Materials

This dissertation explores various nonlinear responses that arise from the rich interplay between quantum geometry, disorder, magnetism and topology in quantum materials. In addition to presenting generalizations of quantum kinetic theory, Kubo formulas and semiclassical Boltzmann transport theory to the nonlinear response regime, we discuss several predictions of novel transport effects and physical insights that emerge from these developments.

==> acknowledgements.tex <==
\begin{acknowledgments}
\end{acknowledgments}

